CABBA: Compatible Authenticated Bandwidth-efficient Broadcast protocol for ADS-B

The Automatic Dependent Surveillance-Broadcast (ADS-B) is a surveillance technology that mandated in many airspaces. It improves safety, increases efficiency and reduces air traffic congestion by broadcasting aircraft navigation data. Yet, ADS-B is vulnerable to spoofing attacks as it lacks mechanisms to ensure the integrity and authenticity of the data being supplied. None of the existing cryptographic solutions fully meet the backward compatibility and bandwidth preservation requirements of the standard. Hence, we propose the Compatible Authenticated Bandwidth-efficient Broadcast protocol for ADS-B (CABBA), an improved approach that integrates TESLA, phase-overlay modulation techniques and certificate-based PKI. As a result, entity authentication, data origin authentication, and data integrity are the security services that CABBA offers. To assess compliance with the standard, we designed an SDR-based implementation of CABBA and performed backward compatibility tests on commercial and general aviation (GA) ADS-B in receivers. Besides, we calculated the 1090ES band's activity factor and analyzed the channel occupancy rate according to ITU-R SM.2256-1 recommendation. Also, we performed a bit error rate analysis of CABBA messages. The results suggest that CABBA is backward compatible, does not incur significant communication overhead, and has an error rate that is acceptable for Eb/No values above 14 dB.

==> Experimentations.tex <==
\section{Backward compatibility experiments} \label{section:experimentalP}

We conducted backward-compatibility tests to verify that the phase overlay
capability, as implemented in CABBA, does not affect the ability of existing
hardware to decode the originals ADS-B messages that are being transmitted in
the in-phase component of the 1090ES carrier.

To do so, we built an SDR-based implementation of CABBA and tested its backward
compatibility with two distinct \textcolor{MidnightBlue}{COTS }ADS-B solutions:
\begin{enumerate}
\item The Appareo Stratus II ADS-B receiver, a non-certified portable device used in general aviation (GA) aircraft.  The Stratus II was connected via Wi-Fi to an IPad running the ForeFlight application displaying ADS-B traffic information.
\item The Collins TSS-4100, a certified avionics device integrating TCAS, transponder and ADS-B traffic surveillance capabilities, used in business jets and airline transport aircraft.  This equipment was connected to a Collins AFD-6520 Adaptative Flight Display to render the traffic information.
\end{enumerate}

The experimental setup we employed involved the following steps:
\begin{enumerate}
\item Generate ADS-B messages and corresponding CABBA packets using custom-made scripts.
\item Generate and transmit the corresponding RF signals using the HackRF One SDR.
\item Receive these RF signals with the corresponding COTS receiver.
\item Check that the transmitted ADS-B information is received and correctly interpreted.  We consider the test to be successful if the transmitted traffic information was displayed with the correct information (call sign, position, etc.).
\end{enumerate}

% Describe scripts
In our experimental setup, the ADS-B messages and the corresponding packets were generated using custom-made scripts.  These scripts are based on the \emph{ADSB\_Encoder.py} \cite{encoder.py} scripts.  This original script only generates ADS-B messages of the position report type, when given the ICAO, latitude, longitude, and altitude of an aircraft as inputs.  However, the logic of ADS-B receivers is such that in order for them to consider a given aircraft's traffic information, they must receive all required ADS-B message types, i.e.~identity, speed, status, and operating status, at the frequency prescribed by the protocol.  Thus, to conduct these tests, we built scripts that generate the remaining types of ADS-B messages\footnote{For this purpose the book \emph{The 1090 Megahertz Riddle} \cite{sun1090mhz} was an invaluable ressource.}.

The scripts we constructed further added the functionality required to generate CABBA messages (keys and certificates) and the corresponding packets.  This includes among others functions to compute the MAC of ADS-B packets, to apply DPSK modulation to data to be transmitted in quadrature, to I-Q modulate the in-phase data in PPM with the quadrature data in DPSK.

For these backward-compatibility experiments, we only constructed and transmitted type A messages, which carry the ADS-B message and its security data.  We did not transmit the other types of CABBA messages (B1, B2 and C), as these would be ignored by legacy receivers since they do not contain ADS-B data.

\begin{figure}[ht] 
\centering
\includegraphics[width=0.98\textwidth]{BacwardCompstratus1.PNG}
\caption{Screen capture of the ForeFlight Maps display with traffic option activated, showing the correct information for the ``synthetic'' aircraft with call sign ``D8PSK'', obtained from an IPad connected to the Stratus II receiver.}
\label{fig:Stratus}
\end{figure}

\begin{figure}[ht] 
  \includegraphics[width=1\textwidth]{BacwardCompCollins1.png}
\caption{Here is a picture of the display AFD-6520 Adaptive Flight Display showing the correct information for the ``synthetic'' aircraft with call sign ``D16PSK''.}
\label{fig:Collins}
\end{figure}

Our tests reveal that CABBA is backward-compatible with the two ADS-in receivers
under test.  Figure \ref{fig:Stratus} shows the display of the ForeFlight
application on the IPAD connected to the Stratus II receiver.  The information
displayed corresponds exactly with the information sent from the Hacker RF One
SDR.  The same is true for the information displayed on the AFD-6520 connected
to the TSS-4100 transponder, as shown in Figure~\ref{fig:Collins}.
%
\textcolor{MidnightBlue}{These results seem to indicate that the use of CABBA with legacy equipment would not compromise safety in the transitional period where some aircraft would not
yet have CABBA-capable ADS-B receivers and displays. This is a very encouraging result that reinforces the assumptions behind the MOPS and our use of it in CABBA.  Further tests should ideally be conducted with a larger set of equipment in laboratory conditions, such as
interoperability and stability tests.  Once these tests are satisfactory,
in-flight tests should follow, ideally in environments with high ADS-B channel
usage and with sources of interference, such as multi-path transmissions due to
terrain (mountains, water surface) or man-made obstacles (buldings, antennae,
etc.).  While we do not think that the use of the MOPS would affect backward
compatibility in such real-world conditions, we do believe that it is important
to study how transmission and bit error rate for the quadrature signal would be
affected by such sources of interference and in high-channel usage.}

\section{Operational Viability of CABBA}
\label{section:experimentalP2}
While CABBA as proposed could provide a high level of security in terms of
message authentication, there are some open questions regarding the viability of
employing it in real-world situations due to operational and technological constraints.  

First, we must determine which modulation scheme is most appropriate, D8PSK or
D16PSK.  Second, we must evaluate the bandwidth overhead of CABBA.  Even with the
use of PSK modulation, CABBA still requires more transmission time than plain
ADS-B.  It thus remains to be seen whether the resulting bandwidth overhead
challenges its use in the already congested 1~090~MHz frequency.  In this
section, we describe our preliminary analysis of these questions using
simulations to evaluate BER and real-world ADS-B data to conduct COR analysis.

\subsection{Comparative BER analysis of CABBA with D8PSK vs.\ D16PSK}
The aim of this BER analysis, is to determine which of the two phase overlay
modulation schemes, D8PSK or D16PSK, provides the best balance between higher
data throughput and acceptable signal quality, i.e.~ADS-B service quality.

The BER is defined as the ratio of erroneously received bits to the total transmitted bits within a designated time frame \cite{ITU-G.821,proakis2008communications}.
It serves as a measure to assess the performance (both in terms of quality and reliability) of a communication system, particularly in digital communication systems where noise and interference can cause errors in the received signal \cite{proakis2008digital}.

We used Simulink \cite{matlab} to model the communication link of the CABBA
protocol.  Then, we used the MATLAB program \texttt{bertool} to perform
Monte-Carlo simulations to determine the BER across an Additive White Gaussian
Noise (AWGN) channel.  

A lower BER indicates a better performance; for ADS-B, the standard establishes
a maximum BER of $10^-6$ \cite{RTCA260C2020}.  The BER curves of the two
implementation of CABBA that we wanted to compare, as well as the BER curves of
the D8PSK, D16PSK, and D32PSK modulations, are depicted in Figure~\ref{fig:BER}.
By observing these curves, we notice that:
\begin{enumerate}
   % \item As expected, CABBA performs better when implemented with D8PSK than when done with D16PSK.
    \item When implemented with D8PSK, CABBA fulfills the requirements of the
      standard for normalized signal-to-noise values (Eb/No) greater than or
      equal to 15 dB.  For these values, the BER is equal to zero, indicating
      that the transmission is error-free.
    \item When implemented using D16PSK, CABBA fails to meet the requirement of
      the standard.
\end{enumerate}

Based on these results, we find that the D8PSK technique is the best method for
implementing phase overlay functionality in avionics systems operating in the
1090ES band.  In the ADS-B context, the D16PSK technique has a significant
impact on data quality and reliability.  Given the high error rates provided by
D16PSK, the increase in throughput may not be worth it.

\begin{figure}[ht] 
\centering
\includegraphics[width=\textwidth]{berCabba.png}
\caption{BER analysis shows that CABBA meets the standard's requirements for
  normalized signal-to-noise values (Eb/No) greater than or equal to 15 dB when
  implemented with D8PSK.  Indeed, the standard requires a BER $< 10^{-6}$ and from
  Eb/No=15 the BER is equal to 0.}
\label{fig:BER}
\end{figure}


\subsection{Channel occupancy rate (COR) analysis}
We conducted a COR analysis to determine to what extent the transmission of
non-standard ADS-B information, which are essential for CABBA support, decreases
the available bandwidth.

The ITU report ITU-R SM.2256-1 \cite{ITU} provides a detailed discussion on
different approaches for measuring and evaluating spectrum occupancy, i.e.~a
methodology to conduct COR analyses.  We used it as a guide to conduct our
analysis.  Indeed, the activity factor ($\gamma$) reflects how active the
communication channel is. It is defined as follows \cite{sun2020analyzing}:
  \begin{equation} \label{eq:activityFactor}
    \gamma = \frac{\sum_{i=1}^{n} \Delta t_i}{\Delta t} 
  \end{equation}

where $\Delta t_i$ represents the channel occupation time for the $i$-th active
transmission and $\Delta t$ represents the total duration of the period being
considered.


We created a baseline of normal 1090ES channel occupancy levels using real ADS-B
data retrieved from the OpenSky Network database \cite{dataset1}. Since 2013, the OpenSky
Network has been gathering continuous air traffic surveillance data as a
non-profit community-based receiver network \cite{Schaefer14a}.  All unfiltered
raw data is kept by OpenSky and made available to academic and institutional
researchers.

To collect data for our research, we chose a receiver near Paris Orly airport
(IATA code \texttt{ORY}, ICAO code \texttt{LFPO}).  We chose this receiver because of the high
density of aircraft traffic that can come within its reception range, including:
\begin{enumerate}
\item Aircraft transiting through the Northern France airspace, i.e.~Paris Area
  Control Center (ACC), one of the busiest aerial corridors in the World.  The
  ADS-B station could receive signals from aircraft at cruise altitude
  (30-35,000 feet) up to 200 nautical miles (360 km).
\item Aircraft transiting through the Paris Terminal Maneuvering Area (TMA)
  that are landing or departing from Paris Charles de Gaulle, Orly or Le
  Bourget, some of the busiest airports in Europe.
  \item Aircraft on the ground at the Orly airport taxiing with transponders
    on.
\end{enumerate}
We obtained a data capture of all traffic for this station for a 24-hour period
on 3 August 2023.  Obviously, aircraft traffic varies during the day, and hence
so does 1090ES transmissions.  We sampled the traffic within each 1-hour period
and observed the transmission rate within 30 second-long periods within that
hour.  Taking six such samples for every hour, we observe quite a bit of
variation in the number of transmissions within each hour; the corresponding
confidence intervals are included in our results below.
\begin{figure}[h]
  \includegraphics[width=1\textwidth]{COR1.PNG}
  \caption{Mean COR for ADS-B transmissions with confidence intervals, computed
    with a sampling of six 30-second periods for every hour of the day, on 3
    August 2023.}
  \label{fig:COR1}
\end{figure}
\begin{table}
%\begin{tabular}{r|cccc}
  \centering
  \begin{tabular}{r||c|c|c|c}
           & Scenario 1 & Scenario 2 & Scenario 3 & Scenario 4 \\
  \hline
  $\Delta_{B1}$ & 5 s    & 5 s     & 5 s   & 5 s \\
  $\Delta_{B2}$ & 5 s    & 10 s   & 10 s   & 15 s \\
  $\Delta_C$   & 5 s    & 15 s    & 20 s   & 30 s
  \end{tabular}
  \caption{Transmission period parameters for each of the four scenarios for
    which we computed the COR values.}
  \label{tab:CABBAparameters}
\end{table}
\begin{figure}[h]
  \includegraphics[width=1\textwidth]{COR2.png}
  \caption{Estimated mean COR values per hour for every hour of 3 August 2023,
    for ADS-B and for CABBA in each of the three possible parameter settings
    described in Table~\ref{tab:CABBAparameters}.}
  \label{fig:COR2}
\end{figure}

\medskip
In CABBA, we transmit four different types of packets, i.e.~packet types A, B1,
B2 and C.  All packets of the same type have the same length and occupy the
channel for the same duration.  Let $\Delta t_A$, $\Delta t_{B1}$, $\Delta
t_{B2}$ and $\Delta t_C$ be the transmission times for each of these packet
types.  These values are proportional to the bit length of these packets
(Table~\ref{tab:CABBApacketTypes}) \emph{plus} the fixed 8-bit preamble.  Given
the 1090ES channel bit rate of 1 megabit/s, this results in 120 ms, 120 ms,
218~ms and 250 ms, respectively.

For each sampled time interval, let $n_A$, $n_{B1}$, $n_{B2}$ and $n_C$ be the
number of packets of each that would be transmitted with CABBA.  The resulting COR value is given by
\begin{equation}
  \gamma = \frac{n_A \, \Delta t_A + n_{B1}\, \Delta t_{B1} + n_{B2} \, \Delta
    t_{B2} + n_C \, \Delta t_C}{\Delta t}
  \label{eq:COR-CABBA}
\end{equation}

For our analysis, we conservatively consider that all aircraft in the dataset
are CABBA-capable and are sending all CABBA packet types as described in the
protocol description in Section~\ref{section:architecture}.  Of course, our
dataset only includes standard ADS-B packets and does not provide us with packet
counts for non-standard CABBA packet type, except for Type A packets for which
the count number $n_A$ is the same as the number of ADS-B packets.  For the
other packet types, we estimate the number of transmissions to be equal to
the number of different aircraft seen in the previous $T$ seconds \cite{Kistan2017}, where $T$ is
the transmission period of that type of packet.
%
For example, let us consider Type B1 packets, i.e.~packets containing unsigned
interval keys.  Each aircraft will send such a packet every $T_{B1}$ seconds,
i.e.~with a $T_{B1}$-second period.  At a given time $t$, let $x$ be the number
of different aircraft (with different ICAO ID) we have seen in our data set in
the previous $T_{B1}$ seconds.  During that time period, some aircraft will have
arrived in range and some others will have departed.  If we assume that within
the sampling interval (30 seconds) both the arrival and departure rate of
aircraft are relatively small and similar to each other, we then can safely
approximate the number of Type B1 packets that will be sent during that period
to be $x$, i.e.~$n_{B1}\approx x$.  The same can be said for the counts $n_{B2}$
of Type B2 and $n_C$ of Type C packets which we approximate to be the number of
different ICAO ID received in the previous $T_{B2}$ and $T_C$ seconds,
respectively.

With these approximations, we are then able to compute the COR value $\gamma$
from Equation~\ref{eq:COR-CABBA}.  We consider four different parameter settings,
described in Table~\ref{tab:CABBAparameters}.  In all scenarios, we keep the same
5-second Tesla interval duration set in SAT.  In the first scenario, Type C
packets are sent at every Tesla interval along with Type B2 packets; Type B1
packets are thus never sent.  This is the ``safest'' scenario in which
CABBA-compatible receivers must wait at most 5 seconds until being able to
authenticate messages, in the sense that the uncertainty period for CABBA
receivers where originators cannot be authenticated is minimized.  The fourth
scenario is the most bandwidth efficient, with Type B2 packets being sent every
other Tesla interval and Type C packet every six intervals.


% Results
%\subsection{Results and Interpretation}
The first finding of this study is that COR values for standard ADS-B vary
between 2.4\% and 9.8\%, for the quietest and busiest hours, 01h00 and 06h00
UTC, i.e.~03h00 and 08h00 Paris local time, respectively. 
%
Second, with respect to CABBA we observe that the maximum overhead corresponds,
obviously, to Scenario 1, with the lowest interarrival times for Type B1, B2 and
C packets.  In Scenario 1, the average overhead in terms of packets transmitted
is 3.76\% per 30-second period, with an observed maximum of 5.76\% during that
day.  In comparison, for the most bandwidth-efficient Scenario~4, the average
overhead is 1.56\% and maximised at 2.38\%.  With respect to channel occupancy
levels observed on that day, this results in a maximum COR increase of 0.43\% of
total bandwidth capacity for the most bandwidth-consuming Scenario 4.  These results are represented graphically in Figure~\ref{fig:COR2}.


In summary, whatever the parameter setting scenario we choose, the
impact of implementing CABBA in terms of bandwidth is negligible.  The
overhead in terms of packets sent is capped at less than 6\%.  This is
in sharp contrast with the original SAT proposal, which has an
estimated overhead of 35\%.

At the observed channel occupation levels, i.e.~COR values between 2\%
and 10\%, the COR increase for CABBA even its most bandwidth-consuming
setting is less than 1\%.  Even in more congested airspaces with
hypothetical COR values of up to 40\%, implementing CABBA would
increase COR to less than 43\%, a very acceptable compromise.

\subsection{Time of uncertainty}

${t}_{uncertainty} = (1 - p - p^2) \frac{T_{{int}}}{2} + p \left(T_{{int}} + \frac{T_{\text{int}}}{2} \right) + p^2 \left(2 T_{{int}} + \frac{T_{{int}}}{2} \right)$



==> TESLAgraph.tex <==
\ifx\du\undefined
  \newlength{\du}
\fi
\setlength{\du}{14\unitlength}
\begin{tikzpicture} [xscale=0.7, yscale=0.7, font=\scriptsize]
\pgftransformxscale{1.000000}
\pgftransformyscale{-1.000000}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\definecolor{dialinecolor}{rgb}{1.000000, 1.000000, 1.000000}
\pgfsetfillcolor{dialinecolor}
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{latex}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw[orange][orange] (4.950000\du,22.850000\du)--(37.750000\du,22.900000\du);
}
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw[orange][orange] (6.500000\du,21.500000\du)--(6.500000\du,24.000000\du);
}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
%\node[anchor=west] at (7.450100\du,23.900000\du){Interval $i-1$};
\node[anchor=west] at (7.05\du,23.900000\du){Interval $i-1$};

% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
%\node[anchor=west] at (15.50\du,23.900000\du){Interval $i$};
\node[anchor=west] at (15.00\du,23.900000\du){Interval $i$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
%\node[anchor=west] at (21.7\du,23.900000\du){Interval $i+1$};
\node[anchor=west] at (21.30\du,23.900000\du){Interval $i+1$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
%\node[anchor=west] at (28.7\du,23.900000\du){Interval $i+2$};
\node[anchor=west] at (28.2\du,23.900000\du){Interval $i+2$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
%\node[anchor=west] at (35.8\du,23.925000\du){time};
\node[anchor=west] at (35.3\du,23.925000\du){time};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (23.100100\du,24.000000\du){};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
%\node[anchor=west] at (8.800000\du,15.600000\du){$K_{ i-1}$};
\node[anchor=west] at (8.400000\du,15.600000\du){$K_{ i-1}$};
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw[orange][orange] (16.3\du,16.990730\du)--(16.300000\du,20.400000\du);
}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
%\node[anchor=west] at (15.425133\du,15.582500\du){$K_{ i}$};
\node[anchor=west] at (15.425133\du,15.582500\du){$K_{ i}$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
%\node[anchor=west] at (22.400000\du,15.600000\du){$K_{ i+1}$};
\node[anchor=west] at (22.000000\du,15.600000\du){$K_{ i+1}$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (29.345200\du,15.582500\du){$K_{ i+2}$};
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsstart{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw[orange] (11.00000\du,15.400000\du)--(15.500000\du,15.400000\du);
}
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (8.605200\du,21.285000\du){$K'_{ i-1}$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (15.5\du,21.505000\du){$K'_{ i}$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (22.427044\du,21.505000\du){$K'_{ i+1}$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (29.725200\du,21.505000\du){$K'_{ i+2}$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (9.800000\du,18.600000\du){$F'(K_{ i-1})$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (16.500000\du,18.600000\du){$F'(K_{ i})$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (23.800000\du,18.600000\du){$F'(K_{ i+1})$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (30.600000\du,18.600000\du){$F'(K_{ i+2})$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (12.00000\du,14.400000\du){$F(K_{ i})$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (18.00000\du,14.400000\du){$F(K_{ i+1})$};
% setfont left to latex
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\node[anchor=west] at (25.500000\du,14.400000\du){$F(K_{ i+2})$};
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw[orange] (9.600000\du,17.000000\du)--(9.6\du,20.409270\du);
}
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw[orange] (23.600000\du,17.000000\du)--(23.6\du,20.409270\du);
}
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsend{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw[orange] (30.50000\du,17.000000\du)--(30.5\du,20.409270\du);
}
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw[orange] (13.625000\du,21.500000\du)--(13.625000\du,24.000000\du);
}
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw[orange] (20.750000\du,21.500000\du)--(20.750000\du,24.000000\du);
}
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw[orange] (27.875000\du,21.500000\du)--(27.875000\du,24.000000\du);
}
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw[orange] (35.000000\du,21.500000\du)--(35.000000\du,24.000000\du);
}
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsstart{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw[orange] (17.000000\du,15.400000\du)--(22.200000\du,15.400000\du);
}
\pgfsetlinewidth{0.050000\du}
\pgfsetdash{}{0pt}
\pgfsetdash{}{0pt}
\pgfsetbuttcap
{
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetfillcolor{dialinecolor}
% was here!!!
\pgfsetarrowsstart{stealth}
\definecolor{dialinecolor}{rgb}{0.000000, 0.000000, 0.000000}
\pgfsetstrokecolor{dialinecolor}
\draw[orange] (24.50000\du,15.400000\du)--(29.0\du,15.400000\du);
}
\end{tikzpicture}


==> architecture.tex <==
\section{CABBA : Compatible Authenticated Bandwidth-efficient Broadcast protocol for ADS-B } \label{section:architecture}

\textcolor{MidnightBlue}{The CABBA solution is presented in this section}. CABBA seamlessly integrates phase-overlay modulation into the ADS-B physical layer and TESLA authentication into its application layer, while using a certificate-based public key infrastructure.  CABBA is based on a new approach in which the fundamental TESLA concept of MAC-based message authentication and key disclosure delay remains intact, while introducing a significant transformation in the way information is transmitted and the type of information transmitted to enhance security. In the following lines, we delve into how CABBA distinguishes itself from previously proposed TESLA-based solutions.


\subsubsection{Integration of Phase Overlay Modulation}
First, we enhance the physical layer of ADS-B by incorporating the phase overlay modulation technique proposed in the patent \cite{EP2661039B1} recently promoted by the RTCA in the most recent version of the ADS-B MOPS \cite{RTCA260C2020}.  As detailed in Figure~\ref{fig:phaseOverlaidFig}, part of the information is conveyed in the in-phase component of the carrier, and the remaining information in its quadrature component.  For this purpose, we consider the two phase overlay modulation techniques mentioned earlier
\begin{enumerate}
  \item the D8PSK method advocated by RTCA \cite{RTCA260C2020}, and
  \item the D16PSK method proposed by academia \cite{Yeste-pskModulation-2015, Zambrano-PSK-2018}.
\end{enumerate}

In order to determine which of these techniques is most appropriate for CABBA, we
first implemented and conducted backward compatibility tests with both of them.
Most importantly, we set to identify which of these modulation techniques
provides an optimum trade-off between higher data throughput and acceptable
quality of signal, i.e.~a lower BER, by conducting a simulation study.  This is
described in Section~\ref{section:experimentalP}.  Nonetheless, since D8PSK is
the proposed standard and for the sake of simplicity of explanation, in the rest
of this section we describe only the implementation with D8PSK.  This
configuration allows for an additional 336 (3*112) bits to be sent together with
the ADS-B 112-bit original message.

\subsubsection{Changes in Packet Structure}
\begin{table*}[ht]
\hskip-1.4cm
\scriptsize 
 \begin{tabular}{|l|l |l |l | l | l | c | c | c| c |}
    \hline
     \multicolumn{4}{|c|}{Type}  & Content & Period & \multicolumn{4}{c|}{Size (bits)} \\\cline{1-4}\cline{7-10}
     \multicolumn{1}{|c|}{TESLA} & \multicolumn{1}{c|}{SAT} & \multicolumn{1}{c|}{SOS} & \multicolumn{1}{c|}{CABBA} & & & \multicolumn{1}{|c|}{TESLA} & \multicolumn{1}{c|}{SAT} & \multicolumn{1}{c|}{SOS} & \multicolumn{1}{c|}{CABBA} \\\hline
%
     A &   &    &   &Message, MAC &  - & - & - & - & - \\ \hdashline
      &  A &    &   &ADS-B message, MAC, sequence no. &  - & - & 136& - & - \\ \hdashline
      &    & A1 &   &ADS-B message &  - & - & - &112 & - \\ 
      &    & A2 &   &MAC & $T_{A2}$ & - & - &128 & - \\ \hdashline
      &    &    & A &ADS-B message, MAC, sequence no. &  - & - & - & - & 112 \\ \hline
    B &    &    &   & Interval key & $T_{B}$  & 128 & - & - & - \\ \hdashline
      &  B &    &   & Interval key & $T_{B}$  & - & 184 & - & - \\ \hdashline
      &    & B  &   & Interval key & $T_{B}$  & - & - & 128 & - \\ \hdashline
      &    &  & B1  & Interval key & $T_{B1}$ & -   & -& -& 128\\ 
      &    &  & B2  & Interval key and signature & $T_{B2}$ & -   & -& - & 210 \\ \hline
      &  C &    &   & \parbox[t]{5cm}{Interval key and signature; \\ aircraft public key and signature} &$T_C$ & - & 1520 & - &-\\ \hdashline
      &    &    &  C &aircraft public key and signature &$T_C$ & - & - & - &242\\ \hline
    \end{tabular}
    
 \caption{A Comparison of CABBA's packet structure with that of earlier TESLA-based solutions. In CABBA, Type B packets are replaced with Type B1 Packets at the beginning of each interval (each $T_B=T_{B1}$ seconds) and by Type B2 packets every $T_{B2}$ seconds.  Type C packets are shorter than in SAT and sent with period $T_C$.}
 \label{tab:CABBApacketTypes}
\end{table*}

The second distinction between CABBA and previous works relates to the content and structure of the packets to be transmitted, as highlighted in Table \ref{tab:CABBApacketTypes}. 

In TESLA, the security information in Type A packets (the MAC) and the interval key subsequently received via Type B packets allows the receiver to verify \emph{data integrity} of the message. \emph{Data origin authentication} is achieved by cross-referencing the information in Type B packets with additional data shared from sender to receiver via a secure communication channel. Both protocols, TESLA \cite{perrig2003tesla} and SOS \cite{sciancalepore2019sos}, assume pre-existing trust between communicating parties, presupposing that the receiver possesses the sender's certificate beforehand. 

In real-life operation, however, an aircraft cannot anticipate precisely which other planes it will encounter along its flight path.  Consequently, the authors of SAT \cite{berthier2017sat} propose a practical solution: distributing certificates through type C packets—an approach we endorse. Nonetheless, there are at least three aviation scenarios in which Bob (the receiver) may not require the certificate, as he may already possess the sender's public key and have duly authenticated its legitimacy. These scenarios are:

\begin{enumerate}
    \item Bob, as an ADS-B ground station, receives messages from aircraft either directly (via Line-of-Sight RF signal) or indirectly (via satellite). To authenticate these messages, Bob's ground station can access a PKI containing public keys of worldwide aircraft, indexed by their ICAO ID. This setup enables instant entity authentication without relying on aircraft to transmit certificates.
    \item Alice, another ADS-B ground station, transmits information to airborne aircraft like Bob through LOS signal. Here, it's reasonable for the aircraft's receiver to hold a small, infrequently updated database of public-key certificates provided by the NAA (e.g., FAA) for authentication.
    \item Air-to-air ADS-B transmissions pose challenges as it's impractical to preload worldwide aircraft public keys into each aircraft's receiver, let alone update them frequently due to aircraft turnover. However, future adoption of integrated digital communications like ATN could enable real-time access to remote PKIs, allowing aircraft to cache recently encountered aircraft's public keys for authentication.
\end{enumerate}


\begin{description}
\item[\textbf{Type A.}] Contain the ADS-B message it MAC and sequence number under the interval
\item[\textbf{Type B1.}] Contain the interval key $K_i$ 
\item[\textbf{Type B2.}] Contain $K_i$ and the digital signature of $K_i$.
\item[\textbf{Type C.}] Contain the aircraft public key $K_{pub}$ and its signature by the CA
\end{description}

Unlike SAT \cite{berthier2017sat}, Type C packets in CABBA do not contain interval key information or interval key signatures, and are therefore shorter. Signed interval keys are transmitted in a new type of packet, Type B2, which contains only an interval key and its signature. This has the advantage that signed keys can be sent with a lower frequency than certificates, resulting in a better use of bandwidth. In addition, this CABBA packet structure has the advantage of reducing bandwidth usage by eliminating the redundant transmissions of the interval keys, as it was the case in SAT \cite{berthier2017sat}.

\subsection{CABBA on the sender side}
CABBA requires airplanes to have a private-public key pair ($K_\text{pr}$, $K_\text{pub}$) and a certificate issued by a well-known and trusted certification authority.  Before the flight begins, Alice, the sender, divides its duration into equal intervals of $d$ seconds, and generates an authentication key for each interval.  The process for generating these keys is the same as that used in TESLA and SAT.  During the flight, the ADS-B messages and their MAC, the authentication keys of the intervals, and the certificate of Alice's aircraft are sent as described below.  

\subsubsection{Sending a message and its MAC}
To send an ADS-B message $m$ at time interval~$i$, Alice first produces the security data $\sigma$ for message $m$. This includes:
\begin{enumerate}
\item The message MAC, formed by the $\lambda$ leftmost bits of the message $\hmac(m,K_i')$
 \item The message sequence number $s$ for $m$ within that interval $i$
\end{enumerate}

In other words $\sigma=\mac \, \| \, s$.
%
%Let $m'$ represent the 120-bit packet containing the 112-bit ADS-B message payload $m$ and the fixed 8-bit preamble.  
As before, this information will continue to be encoded into the in-phase component of the RF signal.  We denote by $P_{A-I}=m$ the message information sent in-phase.  The security information $\sigma$ will be sent using the quadrature component of the RF signal and is thus denoted $P_{A-Q}=\sigma$.

With the same packet length (112 bits) and containing the same information encoded in the same manner as standard ADS-B packets, $P_{A-I}$ packets are intended to be fully intelligible by legacy ADS-B receivers.  A logical packet $P_{A-Q}$, on the other hand, will in principle only be intelligible with CABBA-compliant receivers.  With the choice of D8PSK, the highest quantity of bits that can be encoded in the quadrature component is 336 bits.  Nonetheless, not all of these bits are available to encode the security information $\sigma$.
%
The RTCA recommends using 12 bits to encode a reference phase and 120 parity bits to support the \texttt{RS(54,34)} error-correcting code, which must be applied to the $\sigma$ security data.  This means a maximum size of 204 bits for $\sigma$, which with the 8-bit sequence number $s$ results in a maximum size of 196 bits for the MAC, i.e.~$\lambda\leq 196$.


Alice uses the logical packet $P_{A-I}$ to perform PPM on a pulse train to generate the signal $S_{A-I}(t)$ as follows:
\begin{eqnarray} \label{eq:PPMmod}
  S_{A-I}(t) & = &\sum_{k=0}^{111}g(t-t_k) \quad ; \nonumber \\
  t_k & = & kT_S + m_{t}(1-P_{A-I}(k))
\end{eqnarray}
where $T_S=1\,\mu s$ is the symbol period for 1090ES transmissions,
$m_t=T_S/2$ is the PPM time-modulation index and $P_{A-I}(k)$ is
the value of the $k$-th bit which will be transmitted at time $k*T_S$.
%
Alice simultaneously uses logical packet $P_{A-Q}$ to perform D8PSK modulation on a sine wave to generate the signal $S_{A-Q}(t)$ as follows:
\begin{eqnarray}
  S_{A-Q}(t) &=& \sum_{k=0}^{111}\sin{(\omega_{c}t-\theta_k)} \quad ; \nonumber \\
  \theta_k &=& \frac{2\pi}{8} \; \text{symbol}_{P_{A-Q}}(k)  \label{eq:DPSKmod}
\end{eqnarray}
%
where $\omega_c$ represents the carrier signal frequency, $\theta_k$ is the phase associated to the 8PSK symbol $\text{symbol}_{P_{A-Q}}(k) \in [0,7]$, which is computed from the three bits from $P_{A-Q}$ to be transmitted at time $k*T_S$. 

\begin{equation}
\begin{split}
\text{symbol}_{P_{A-Q}}(k) = & 2^2P_{A-Q}(3k) + 2^1P_{A-Q}(3k+1) +\\
& 2^0P_{A-Q}(3k+2)
\end{split}
\end{equation}

These two signals $S_{A-I}$(t) and $S_{A-Q}$(t) are then used by Alice
to I-Q modulate (Equation~\ref{eq:IQmod}) the 1090ES carrier and so,
produce the radio signal $S_A$ to be broadcast.
\begin{equation} \label{eq:IQmod}
    S_A(t)=S_{A-I}(t)\cos(\omega_{c}t) + S_{A-Q}(t)\sin(\omega_{c}t)
\end{equation}

\begin{figure*}[t!] 
\centering
\includegraphics[width=0.9\textwidth]{PA.pdf}
\caption[Structure of the Type A packets in CABBA.]{Structure of the Type A packets in CABBA.  The ADS-B message $m$ encoded in the in-phase component $P_{A-I}$ (in this example an airborne position report) and the security data $\sigma$ in the quadrature component $P_{A-Q}$.  These two logical packets are then used to generate the in-phase and quadrature signal components $S_{A-I}$ and $S_{A-Q}$ of the RF signal to be transmitted $S_{A}$.}\label{fig:PA}
\end{figure*}
  
\subsubsection{Sending authentication keys and their signatures}
In order to allow the receiver to authenticate the Type A messages sent in interval $i$, the sender must later disclose the corresponding interval keys and their signatures.  This is done by sending Type B1 and B2 packets in subsequent intervals.  

Type B1 packets contain the TESLA interval $K_i$ (128 bits) from which the authentication key $K_i'=F'(K_i)$ of the interval $i$ is calculated.  The corresponding packet $P_{B1}$ will be transmitted during the next time interval $i+1$.  These packets are sent at the beginning of each interval, i.e.~every $T_{B1}=T_{int}$ seconds.

The signature of the authentication keys is added in Type B2 packets.  B2 packets replace B1 packets at the beginning of the interval, every fixed number $k$ of intervals.  Their transmission period $T_{B2}$ is thus a multiple of $T_{B1}$, with $T_{B2}=kT_{B1}$.  A typical packet $P_{B2}$ of this type will contain:
\begin{equation}
P_{B2} = K_i \, \| \, \sig_{K_{pr}}(K_i)
\end{equation}
where the $\sig_{K_{pr}}$ represents the chosen signature-generating function with private key $K_{pr}$.  

For Type B1 packets, the logical information $P_{B1}$ is split between packets $P_{B1-I}$ and $P_{B1-Q}$ that will be transmitted through the in-phase and quadrature components of the RF signal.  The in-phase packet $P_{B1-I}$ contains the 50 leftmost bits of the $K_I$ and the quadrature packet $P_{B1-Q}$ contains the remaining 78 bits, as indicated in Figure~\ref{fig:PB1}. 

For Type B2 packets, the information is similarly split into packets $P_{B2-I}$ and $P_{B2-Q}$.  The in-phase component $P_{B2-I}$ contains the entire interval key $K_i$ and the leftmost 14 bits of the signature, while the quadrature component $P_{B2-Q}$ contains the remaining 498 bits of the 512-bit signature.  

The signal components $S_{B1-I}$, $S_{B1_Q}$, $S_{B2-I}$ and $S_{B2-Q}$ are then generated similarly as for Type A packets (Equations~\ref{eq:PPMmod}, \ref{eq:DPSKmod} and \ref{eq:IQmod}).

\begin{figure*}[t]

\begin{subfigure}{\textwidth}
\centering
  \includegraphics[clip,width=0.9\textwidth]{PB1.pdf}
  \caption{Structure of Type B1 packets, 112 bits for $P_{B1-I}$ and 336 bits $P_{B2-Q}$}\label{fig:PB1}
\end{subfigure}
\begin{subfigure}{\textwidth}
\centering
  \includegraphics[clip,width=0.9\textwidth]{PB2.pdf}
  \caption{Structure of Type B2 packets, 210 bits for $P_{B2-I}$ and 630 bits $P_{B2-Q}$}\label{fig:PB2}
\end{subfigure}
\caption{Structure of Type B1 and B2 packets, conveying only the authentication key or the authentication key and its signature, respectively.}\label{fig:PB}
\end{figure*}


\subsubsection{Sending the certificate of the transmitting aircraft}
Alice will broadcast the certificate of aircraft every $T_C$ seconds.  The Type C packet $P_C$ contains the public key of the aircraft $K_{pub}$ and the signature of this key $\sig_{K_{prCA}}(K_{pub})$.  With a security strength of 128 bits, an ECDSA public key size of 256 bits is required, resulting in a signature size of 512 bits \cite{FIPS186-5}.  The first 181 bits of the public key $K_{pub}$ are encoded in the in-phase packet $P_{C-I}$ and the remaining 75 bits at the beginning of the quadrature packet $P_{C-Q}$.  The 512 bits of the signature $\sig$ are also encoded into $P_{C-Q}$.

After encoding $P_{C-I}$ and $P_{C-Q}$, the sender generates the signals $S_{ C-I}$, $S_{C-Q}$, and finally the signal $S_C$ which she broadcast.  The procedure for producing these signals is the same as for producing signals for Type A and B packets.

\begin{figure*}[t]
\centering
\includegraphics[width=0.9\textwidth]{PC.pdf}
\caption{Structure of Type C packets.  They contain the public key $K_{pub}$ of the aircraft and the signature of said key $\sig_{K_{prCA}}(K_{pub})$.  These packets are then used to generate the transmitted signal $S_C$.}\label{fig:PC}
\end{figure*}

\subsection{CABBA on the receiver side}
\begin{figure}[h] 
\centering
\includegraphics[width=0.8\textwidth]{stateDiagramRX.pdf}
\caption{State diagram illustrating the authentication process for ADS-B messages on the receiver side.}
\label{fig:Methodology}
\end{figure}

\subsubsection{Reception and demodulation of signals}
The process of receiving and demodulating messages by Bob (the receiver) is the same for all packet types.  The received signal $S$ is first demodulated with quadrature local oscillators to obtain the in-phase component $S_I$ and the quadrature component $S_Q$.  Bob then performs PPM demodulation onto $S_I$ and D8PSK demodulation onto $S_Q$, to generate logical packets $P_I$ and $P_Q$,
respectively.  Depending on the format of these packets, Bob determines the original packet type (A, B1, B2 or C) and processes them accordingly.  The processing of the CABBA messages contained within these logical packets is detailed below and depicted in the state diagram in Figure~\ref{fig:Methodology}.

\subsubsection{Processing the ADS-B message and its security data}
As described above, the ADS-B message information and its security data is contained in Type A packet $P_{A-I}$ and $P_{A-Q}$, respectively.  Bob thus extracts the message $m'$ from $P_{A-I}$ and the security data $\sigma$ (its sequence number $s$ and the MAC) from $P_{A-Q}$.  Lastly, he stores the triplet $(m',s,\mac)$ in a buffer until he can verify the integrity of the message.

\subsubsection{Verification of security properties}

CABBA is an asynchronous protocol and there is no guarantee that messages corresponding to a particular aircraft will be received in any particular order. The state diagram in Figure~\ref{fig:Methodology} describes the various states in which the receiver of CABBA could be depending on what security information, i.e.~what CABBA packet types, have been received so far.  Note that such a state diagramme is used for all messages received with the same ICAO ID, i.e.~purportedly corresponding to the same aircraft.

% NAMES OF STATES
% S_0: Initial state
% S_1: Interval key received
% S_2: Signed interval key received
% S_3: Certificate received
% S_4: Authentication

The state machine is initialized at state $S_0$ when the first packet for a given ICAO ID is received.  If it is a Type A packet, it will be stored and the machine stays in the same state.  Reception of type B1 packet containing an interval key will generate a transition to State $S_1$.  Reception of a Type B2 packet, a \emph{signed} interval key,  will make the state machine transition to State $S_2$.  Finally, the (unlikely but possible) reception of a certificate in a Type C packet before a Type B1 or B2 packet will transition to State $S_3$. In all of these states ($S_1$, $S_2$ and $S_3$), subsequent reception of ADS-B messages in Type A packets and further interval keys in Type B packets causes no transitions.

At this point, the receiver is unable to perform neither entity authentication nor data origin authentication of any messages received because some security information is missing (has not been received), i.e.~either a validate certificate in the case of State $S_2$, a signed interval key in the case of State $S_3$, or both in State $S_1$.  Nonetheless, the receiver is able to perform data integrity verification of the ADS-B messages received in previous intervals.

% Data integrity verification
\paragraph{Data Integrity}
In order to validate the message integrity of a message $m'$ received during interval $i$, Bob must have already received Type B1 packets $P_{B1-I}$ and $P_{B1_Q}$ at the beginning of the next interval $i+1$.  From these packets he will be able to reconstruct the interval key $K_i$ by concatenating the first 50 bits contained in $P_{B1-I}$ and the remaining 78 bits contained in $P_{B1-Q}$
(as shown in Figure~\ref{fig:PA}).  The next step is to calculate the authentication key $K_i'=F'(K_i)$.  Then, Bob calculates the ``correct'' HMAC of the received message $m'$ with this authentication key $K_i'$ as follows
$\hmac' = \hmac(m',K_i')$. Finally, Bob compares the $\lambda$ leftmost bits of $\hmac'$ with the received $\mac$.  If they coincide, Bob will accept the message $m'$, otherwise, he will ignore it.

Note that this verification only meets the goal of \emph{data integrity} of the message $m'$, i.e.~that the message has not been modified after its MAC was computed by its originator, whomever the originator might be (friend or foe, real aircraft or hacker).

%Same origin discrimination
\paragraph{Same-origin discrimination}
While in States $S_1$, $S_2$ and $S_3$ the receiver is unable to perform data
origin authentication, there is an important security property that can be asserted at
this point: \emph{same-origin discrimination}, i.e.~the ability to determine
which message was sent by which sender, without necessarily having authenticated
them.

To better understand this property, consider the following spoofing scenario.
The attacker is aware that Alice's aircraft with ICAO ID $X_A$ is currently
broadcasting ADS-B messages that Bob is receiving.  The intent of the spoofer is
to send  counterfeit ADS-B messages bearing the same ICAO ID $X_A$.  Aware that the
aircraft ADS-B transmitter and the receiver have implemented CABBA, the spoofer
can generate his own interval key sequence and use it to authenticate his fake
messages.  More precisely, let $K^*=K^*_0,\ldots,K^*_N$ be the interval sequence
generated by the aircraft and let $K^\dag=K^\dag_0,\ldots,K^\dag_N$ be the
sequence generated by the spoofer.  The spoofer then generates his own messages,
including hashes computed with his own key sequence.

If both spoofer and Alice's aircraft are in Bob's reception range, Bob would
then receive these two message streams corresponding to the same ICAO ID $X_A$,
potentially contradictory.  Thus, while Bob may not be able to know which
messages came from the spoofer or from Alice's aircraft, he will, nonetheless,
be able to correctly associate a new message $m'$ to either stream.  Consider
two messages $m_1$ and $m_2$ received by Bob at intervals $i_1$ and $i_2$,
$i_2>i_1$, respectively, and whose integrity was verified by Bob in the
subsequent intervals $i_1+1$ and $i_2+1$ with interval keys $K_{i_1}$ and
$K_{i_2}$, respectively. Then if:
\begin{equation}
K_{i_1}=F^{(i_2-i_1)}(K_{i_2})
\end{equation}
then Bob knows that $m_1$ and $m_2$ were sent by the same sender.
In other words, in the above scenario Bob will be able to detect
that there are two different senders $A^*$ and $A^\dag$ sending messages with
the same ICAO code, and further know which message corresponds to which sender.
He will not, however, know which one corresponds to the real aircraft $A$.

\paragraph{Authentication}
%Data origin authentication
When Bob has received all required security information, i.e.~a signed interval key and a certificate, he can then perform both identity authentication of the sender and message authentication (i.e.~data origin authentication) of previously received messages.  This will be possible when the state machine transitions to State $S_4$.\\

%Identity authentication
\textbf{Identity Authentication} Upon receiving Type C packet $P_{C-I}$ and $P_{C-Q}$, the public key $K_{\text{pub}}$ is extracted by concatenating the 181 bits in $P_{C-I}$ and the first 75 bits in $P_{C-Q}$.  The key signature $\sig_{K_{prCA}}(K_{pub})$ is
extracted from the remaining 512 bits of $P_{C-Q}$, as shown in Figure~\ref{fig:PC}.  Since Bob knows the public key $K_{pubCA}$ of the
Certificate Authority, he is able to verify the validity of the signature of the aircraft key the corresponding signature verification procedure \texttt{Verify}, that returns a boolean of \texttt{true} if the signature is valid.  In other
words, let $v_1$ be the result of this first signature verification:
\begin{equation} \label{eq:v1}
v_1= \texttt{Verify}(K_{pubCA},\sig_{K_{prCA}}(K_{pub}),K_{pub})
\end{equation}

%Interval key authentication
\textbf{Message authentication} Finally, having received a Type B2 packet $P_{B2-I}$ and $P_{B2-Q}$, Bob proceeds to extract the key $K_i$ from $P_{B2-I}$. To obtain the signature $\sig_{K_{pr}}(K_i)$, he concatenates the 14 bits from $P_{B2-I}$ with the 498 bits from $P_{B2-Q}$. Using this information, Bob verifies the authenticity of the interval key $K_i$. Let $v_2$ be the result of this verification procedure, as defined by the equation:
\begin{equation} \label{eq:v2}
v_2= \texttt{Verify}(K_{pub},\sig_{K_{pr}}(K_i),K_i)
\end{equation}
If $v_2$ evaluates \texttt{true}, it means that the key $K_i$ is authentic, i.e. that it has been generated by  Alice. Furthermore, this outcome also implies that all ADS-B messages for which the $\mac$ has been computed using $K_i$ can also be deemed authentic.


==> operational2.tex <==
\section{Operational Viability of CABBA}
\label{section:experimentalP2}
While CABBA as proposed could provide a high level of security in terms of
message authentication, there are some open questions regarding the viability of
employing it in real-world situations due to operational and technological constraints. 

First, we must determine which modulation scheme is most appropriate, D8PSK or
D16PSK.  Second, we must evaluate the bandwidth overhead of CABBA.  Even with the
use of PSK modulation, CABBA still requires more transmission time than plain
ADS-B.  It thus remains to be seen whether the resulting bandwidth overhead
challenges its use in the already congested 1~090~MHz frequency.
% New phrase, added for subsection 7.3 at request of reviewer
Finally, we explore the impact on aviation safety of the fact that not
all CABBA messages can be authenticated instantaneously.
%
%% In this
%% section, we describe our preliminary analysis of these questions using
%% simulations to evaluate BER and real-world ADS-B data to conduct COR analysis.

\subsection{Comparative BER analysis of CABBA with D8PSK vs.\ D16PSK}
The aim of this BER analysis, is to determine which of the two phase overlay
modulation schemes, D8PSK or D16PSK, provides the best balance between higher
data throughput and acceptable signal quality, i.e.~ADS-B service quality.

The BER is defined as the ratio of erroneously received bits to the total transmitted bits within a designated time frame \cite{ITU-G.821,proakis2008communications}.
It serves as a measure to assess the performance (both in terms of quality and reliability) of a communication system, particularly in digital communication systems where noise and interference can cause errors in the received signal \cite{proakis2008digital}.

We used Simulink \cite{matlab} to model the communication link of the CABBA
protocol.  Then, we used the MATLAB program \texttt{bertool} to perform
Monte-Carlo simulations to determine the BER across an Additive White Gaussian
Noise (AWGN) channel. 

A lower BER indicates a better performance; for ADS-B, the standard establishes
a maximum BER of $10^-6$ \cite{RTCA260C2020}.  The BER curves of the two
implementation of CABBA that we wanted to compare, as well as the BER curves of
the D8PSK, D16PSK, and D32PSK modulations, are depicted in Figure~\ref{fig:BER}.
By observing these curves, we notice that:
\begin{enumerate}
   % \item As expected, CABBA performs better when implemented with D8PSK than when done with D16PSK.
    \item When implemented with D8PSK, CABBA fulfills the requirements of the
      standard for normalized signal-to-noise values (Eb/No) greater than or
      equal to 15 dB.  For these values, the BER is equal to zero, indicating
      that the transmission is error-free.
    \item When implemented using D16PSK, CABBA fails to meet the requirement of
      the standard.
\end{enumerate}

Based on these results, we find that the D8PSK technique is the best method for
implementing phase overlay functionality in avionics systems operating in the
1090ES band.  In the ADS-B context, the D16PSK technique has a significant
impact on data quality and reliability.  Given the high error rates provided by
D16PSK, the increase in throughput may not be worth it.

\begin{figure}[ht]
\centering
\includegraphics[width=\textwidth]{berCabba.png}
\caption{BER analysis shows that CABBA meets the standard's requirements for
  normalized signal-to-noise values (Eb/No) greater than or equal to 15 dB when
  implemented with D8PSK.  Indeed, the standard requires a BER $< 10^{-6}$ and from
  Eb/No=15 the BER is equal to 0.}
\label{fig:BER}
\end{figure}


\subsection{Channel occupancy rate (COR) analysis}
We conducted a COR analysis to determine to what extent the transmission of
non-standard ADS-B information, which are essential for CABBA support, decreases
the available bandwidth.

The ITU report ITU-R SM.2256-1 \cite{ITU} provides a detailed discussion on
different approaches for measuring and evaluating spectrum occupancy, i.e.~a
methodology to conduct COR analyses.  We used it as a guide to conduct our
analysis.  Indeed, the activity factor ($\gamma$) reflects how active the
communication channel is. It is defined as follows \cite{sun2020analyzing}:
  \begin{equation} \label{eq:activityFactor}
    \gamma = \frac{\sum_{i=1}^{n} \Delta t_i}{\Delta t}
  \end{equation}

where $\Delta t_i$ represents the channel occupation time for the $i$-th active
transmission and $\Delta t$ represents the total duration of the period being
considered.


We created a baseline of normal 1090ES channel occupancy levels using real ADS-B
data retrieved from the OpenSky Network database \cite{dataset1}. Since 2013, the OpenSky
Network has been gathering continuous air traffic surveillance data as a
non-profit community-based receiver network \cite{Schaefer14a}.  All unfiltered
raw data is kept by OpenSky and made available to academic and institutional
researchers.

To collect data for our research, we chose a receiver near Paris Orly airport
(IATA code \texttt{ORY}, ICAO code \texttt{LFPO}).  We chose this receiver because of the high
density of aircraft traffic that can come within its reception range, including:
\begin{enumerate}
\item Aircraft transiting through the Northern France airspace, i.e.~Paris Area
  Control Center (ACC), one of the busiest aerial corridors in the World.  The
  ADS-B station could receive signals from aircraft at cruise altitude
  (30-35,000 feet) up to 200 nautical miles (360 km).
\item Aircraft transiting through the Paris Terminal Maneuvering Area (TMA)
  that are landing or departing from Paris Charles de Gaulle, Orly or Le
  Bourget, some of the busiest airports in Europe.
  \item Aircraft on the ground at the Orly airport taxiing with transponders
    on.
\end{enumerate}
We obtained a data capture of all traffic for this station for a 24-hour period
on 3 August 2023.  Obviously, aircraft traffic varies during the day, and hence
so does 1090ES transmissions.  We sampled the traffic within each 1-hour period
and observed the transmission rate within 30 second-long periods within that
hour.  Taking six such samples for every hour, we observe quite a bit of
variation in the number of transmissions within each hour; the corresponding
confidence intervals are included in our results below.
\begin{figure}[h]
  \includegraphics[width=1\textwidth]{COR1.PNG}
  \caption{Mean COR for ADS-B transmissions with confidence intervals, computed
    with a sampling of six 30-second periods for every hour of the day, on 3
    August 2023.}
  \label{fig:COR1}
\end{figure}
\begin{table}
%\begin{tabular}{r|cccc}
  \centering
  \begin{tabular}{l||c|c|c|c}
           & Scenario 1 & Scenario 2 & Scenario 3 & Scenario 4 \\
  \hline
  $T_{B1}$ & 5 s    & 5 s     & 5 s   & 5 s \\
  $T_{B2}$ & 5 s    & 10 s   & 10 s   & 15 s \\
  $T_C$   & 5 s    & 15 s    & 20 s   & 30 s
  \end{tabular}
  \caption{Transmission period parameters for each of the four scenarios for
    which we computed the COR values.}
  \label{tab:CABBAparameters}
\end{table}
\begin{figure}[h]
  \includegraphics[width=1\textwidth]{COR2.png}
  \caption{Estimated mean COR values per hour for every hour of 3 August 2023,
    for ADS-B and for CABBA in each of the three possible parameter settings
    described in Table~\ref{tab:CABBAparameters}.}
  \label{fig:COR2}
\end{figure}

\medskip
In CABBA, we transmit four different types of packets, i.e.~packet types A, B1,
B2 and C.  All packets of the same type have the same length and occupy the
channel for the same duration.  Let $\Delta t_A$, $\Delta t_{B1}$, $\Delta
t_{B2}$ and $\Delta t_C$ be the transmission times for each of these packet
types.  These values are proportional to the bit length of these packets
(Table~\ref{tab:CABBApacketTypes}) \emph{plus} the fixed 8-bit preamble.  Given
the 1090ES channel bit rate of 1 megabit/s, this results in 120 ms, 120 ms,
218~ms and 250 ms, respectively.

For each sampled time interval, let $n_A$, $n_{B1}$, $n_{B2}$ and $n_C$ be the
number of packets of each that would be transmitted with CABBA.  The resulting COR value is given by
\begin{equation}
  \gamma = \frac{n_A \, \Delta t_A + n_{B1}\, \Delta t_{B1} + n_{B2} \, \Delta
    t_{B2} + n_C \, \Delta t_C}{\Delta t}
  \label{eq:COR-CABBA}
\end{equation}

For our analysis, we conservatively consider that all aircraft in the dataset
are CABBA-capable and are sending all CABBA packet types as described in the
protocol description in Section~\ref{section:architecture}.  Of course, our
dataset only includes standard ADS-B packets and does not provide us with packet
counts for non-standard CABBA packet type, except for Type A packets for which
the count number $n_A$ is the same as the number of ADS-B packets.  For the
other packet types, we estimate the number of transmissions to be equal to
the number of different aircraft seen in the previous $T$ seconds \cite{Kistan2017}, where $T$ is
the transmission period of that type of packet.
%
For example, let us consider Type B1 packets, i.e.~packets containing unsigned
interval keys.  Each aircraft will send such a packet every $T_{B1}$ seconds,
i.e.~with a $T_{B1}$-second period.  At a given time $t$, let $x$ be the number
of different aircraft (with different ICAO ID) we have seen in our data set in
the previous $T_{B1}$ seconds.  During that time period, some aircraft will have
arrived in range and some others will have departed.  If we assume that within
the sampling interval (30 seconds) both the arrival and departure rate of
aircraft are relatively small and similar to each other, we then can safely
approximate the number of Type B1 packets that will be sent during that period
to be $x$, i.e.~$n_{B1}\approx x$.  The same can be said for the counts $n_{B2}$
of Type B2 and $n_C$ of Type C packets which we approximate to be the number of
different ICAO ID received in the previous $T_{B2}$ and $T_C$ seconds,
respectively.

With these approximations, we are then able to compute the COR value $\gamma$
from Equation~\ref{eq:COR-CABBA}.  We consider four different parameter settings,
described in Table~\ref{tab:CABBAparameters}.  In all scenarios, we keep the same
5-second Tesla interval duration set in SAT.  In the first scenario, Type C
packets are sent at every Tesla interval along with Type B2 packets; Type B1
packets are thus never sent.  This is the ``safest'' scenario in which
CABBA-compatible receivers must wait at most 5 seconds until being able to
authenticate messages, in the sense that the uncertainty period for CABBA
receivers where originators cannot be authenticated is minimized.  The fourth
scenario is the most bandwidth efficient, with Type B2 packets being sent every
other Tesla interval and Type C packet every six intervals.


% Results
%\subsection{Results and Interpretation}
The first finding of this study is that COR values for standard ADS-B vary
between 2.4\% and 9.8\%, for the quietest and busiest hours, 01h00 and 06h00
UTC, i.e.~03h00 and 08h00 Paris local time, respectively.
%
Second, with respect to CABBA we observe that the maximum overhead corresponds,
obviously, to Scenario 1, with the lowest interarrival times for Type B1, B2 and
C packets.  In Scenario 1, the average overhead in terms of packets transmitted
is 3.76\% per 30-second period, with an observed maximum of 5.76\% during that
day.  In comparison, for the most bandwidth-efficient Scenario~4, the average
overhead is 1.56\% and maximised at 2.38\%.  With respect to channel occupancy
levels observed on that day, this results in a maximum COR increase of 0.43\% of
total bandwidth capacity for the most bandwidth-consuming Scenario 4.  These results are represented graphically in Figure~\ref{fig:COR2}.


In summary, whatever the parameter setting scenario we choose, the
impact of implementing CABBA in terms of bandwidth is negligible.  The
overhead in terms of packets sent is capped at less than 6\%.  This is
in sharp contrast with the original SAT proposal, which has an
estimated overhead of 35\%.

At the observed channel occupation levels, i.e.~COR values between 2\%
and 10\%, the COR increase for CABBA even its most bandwidth-consuming
setting is less than 1\%.  Even in more congested airspaces with
hypothetical COR values of up to 40\%, implementing CABBA would
increase COR to less than 43\%, a very acceptable compromise.

\subsection{Safety Impact of Unauthenticated Messages}

%Summary
%1. In terms of aviation safety, the important measure is time of uncertainty
%2. Case analysis: TCAS vs. ATC (and subcases)
%3. Conclusion: in all cases, time of uncertainty is acceptable
%4. Only unauthenticated packets left are legacy ADS-B packets in transition situations

\textcolor{MidnightBlue}{
The key idea in TESLA that enables authenticated broadcast is the \emph{delayed} key disclosure.  However, this feature introduces a safety trade-off: messages cannot be immediately authenticated, resulting in an \emph{uncertainty delay}
$\Delta_u$ between message arrival and authentication.
%
As discussed in Section~\ref{sec:CABBA-rcv}, in order to authenticate a message the following information must be in possession of the receiver: 1) the interval key for that message, 2) a signed interval key from this or a previous interval, and 3) the sender's certificate.  This information may have already been received in Type B1, B2 or C packets.   While the delay of arrival of such information is bounded by their respective interarrival periods, their order of arrival at the receiver is non-deterministic and thus the actual value of $\Delta_u$  is also non-deterministic.
%
Further analysis of what these uncertainty delays are, and what is their impact on aviation safety, depends on what application and what context the ADS-B information is being used in.  We analyze various scenarios in TCAS and ATC application below.
}

\subsubsection{Impact of packet loss on uncertainty delay}
\textcolor{MidnightBlue}{
In addition, we have to consider packet loss from noise, interference,
or collisions due to congestion, which could introduce a further delay
due to having to wait and additional 1 or~2 subsequent periods.  The
following equation describes an approximation of the expected value of $\Delta_u$ as a function of probability of packet loss $p$ and the interarrival period $T$ of the required information, where the first term corresponds to the packet being successfully received in the first interval, the second term in the second interval, etc.%
}
\begin{eqnarray}\label{delta-u}
  \overline{\Delta_u} & = & (1 - p - p^2) \frac{T}{2} + p  \left( T + \frac{T}{2} \right) +
  p^2 \left(2T + \frac{T}{2} \right) \nonumber \\
  & = & \frac{T}{2} (1+2p+4p^2)
\end{eqnarray}

\textcolor{MidnightBlue}{Previous works \cite{Schaefer14a,sciancalepore2019reliability} have explored the packet loss ratio for ADS-B. They apply a conservative definition, where packet loss occurs if \emph{any} receiver within the aircraft's range is missing the corresponding reception record.  In the rest of this section, we approximate the probability of packet loss at a particular receptor, by interpolating from the empirical cumulative distribution function between packet loss and distance in \cite{sciancalepore2019reliability}.}

\textcolor{MidnightBlue}{
\subsubsection{Uncertainty Delays in TCAS}
TCAS technology is essential in two environments: 1) non-radar environments, like oceanic regions, where ATC may be unable to provide separation services, and 2) dense traffic areas, such as busy airport terminals, where separation conflicts are likely to occur.  The TCAS standards and supporting equipment ensure pilots have sufficient situational awareness of nearby aircraft within predefined \emph{protection volumes}.  These volumes are defined to address potential separation conflicts within specific \emph{time} periods: 20--48 seconds for traffic advisories (TA) and 15--35 seconds for resolution advisories (RA).  These intervals provide pilots with adequate time to enhance their situational awareness of incoming traffic (TA) and to execute evasive maneuvers (RA). It is thus very important that uncertainty delays do not significantly reduce the reaction time for pilots.}

  For aircraft in flight, the line-of-sight range corresponds to the distance to the horizon.  For typical altitudes that are small in comparison with the radius of the Earth, this can be approximated as follows:
  \begin{equation}
    \text{LOS range (in NM)}=1.06*\sqrt{\text{altitude (in feet)}}
  \end{equation}

  In remote and oceanic areas, TCAS establishes a maximum lateral closure rate of 1~200 knots (1~200 nautical miles (NM) per hour= 2~222 km/h), resulting in protected volumes with radii of 16 NM for TA and 11,6 NM for RA (distances corresponding to this closure velocity and the specified time periods for TA and RA).
%
  At a cruise altitude of 35~000 feet, the line-of-sight (LOS) range between aircraft is approximately 458 NM, providing 22,9 minutes of transmission time before the aircraft enters the protected volume.  In terminal areas, arriving aircraft typically operate between 10~000 and 3~000 feet, resulting in a worst-case minimum LOS range of 134,2 NM (both at 3~000 feet).  With a speed limit of 250 knots and a maximum closure rate of 500 knots, these aircraft will enter LOS range at least 16,1 minutes before entering each other's protected volumes. 
%
In both cases, this is significantly larger than the proposed $T_{B2}$ and $T_C$ periods, which guarantees reception of the required Type B1 and C packets, with high probability, even accounting for the packet loss rates at those distances.  Thus, the only significant delay to be considered is that due the delayed transmission of the interval keys ($T_{B1}$).

At distances conmesurate with the radii of protected volumes, the
probability of packet loss for Type B1 packets is modest and the
resulting expected value of $\Delta_u$ is less than 3,0 s, for both TA
and RA.  In other words, the use of CABBA reduces reaction time by at
most 3 s, which we deem acceptable compared with the above-mentioned
overall reaction times for TA and RA protected volumes.

\begin{table}[ht]
    \hskip-1.7cm
    \begin{tabular}{|c||c|c|c|c||c|c|}%{|l|l|c|c|c|}
      \hline
      \textbf{TCAS} & \textbf{radius} & $p$ (\%) & $\Delta_u(T_{B1})$ (s) & \textbf{time} (s)& \textbf{LOS} (min) &$\Delta_u(T_C)$ (s)\\
      \hline
        TA & 6,6--16 NM  & 8,9 & 3,0 & 20--48   & 16,1--22,9 & 18,1 \\
           & (12,2--29,6 Km) & & & & & \\
        \hline
        RA & 5--11,6 NM  & 6,4 & 2,9& 15--35 & 16,1--22,9 & 17,2 \\
           & (9,3--21,5 Km) & & & & & \\
        \hline
    \end{tabular}
    \caption{Packet loss probability and uncertainty times for TCAS.  We give the \emph{radius} for the corresponding protected volume, the derived probability $p$ of packet loss at that distance (as per \cite{sciancalepore2019reliability}), the resulting expected authentication delay due to interval key transmission $\Delta_u(T_{B1})$, and compare it with the total reaction time as per the TCAS standard \cite{TCAS}.  In addition, we compare the time in the LOS range %% for both aircraft within a terminal area (3 to 10~000 feet, max 500 knots closure rate) and at cruise altitude (35~000 feet, max 1~200 knots closure rate),
      and compare it with the expected uncertainty delay for transmission of Type C packets $\Delta_u(T_c)$.  Here, we use the parameters for the ``worst-case'' Scenario 4 of Table~\ref{tab:CABBAparameters}, i.e.~$T_{B1}=5$ s and $T_{B2}=T_C=30$ s.}
    \label{tab:packetloss}
\end{table}

\subsubsection{Uncertainty Delays in ATC}
\textcolor{MidnightBlue}{In ATC, air traffic controllers utilize interconnected air traffic management (ATM) systems that can communicate with airborne aircraft via digital channels (e.g.~ACARS, CPDLC). It is reasonable to expect that these systems will have access to a PKI with aircraft certificates or receive them along with flight plan information.  The same can be said of signed keys for the initial interval of a flight, that could be transmitted by the aircraft at the gate.  In this case, the primary factor affecting uncertainty delays woul be the interarrival time of interval keys, i.e.~the parameter $T_{B1}$.}

%%% MIKAELA: RECALCULA TODAS LAS DISTANCIAS LOS Y TIEMPOS ANTES DE ESTO

\textcolor{MidnightBlue}{If the certificate or signed key is unavailable, then the ATM system may have to rely on their transmission by CABBA through Type B1 and C2 packets, with the correspoding authentication uncertainty delay.  The impact of this uncertainty will depend on the type and size of airspace being controlled.
  \begin{description}
  \item[Airport control zones (aka ``Tower'').] A sector centered on an airport, with a typical radius of 5 NM and maximum altitude of 3~000 fet.
  \item[Terminal areas.] A inverted-cone shaped sector above the control zone, with up to 40 NM in radius and up to 12~500 feet.
    \item[Area Control Center.] A large sector, covered by surveillance from a single surveillance installation (radar or ADS-B receiver), typically with a 100--150 NM radius, in order to ensure that all aircraft in the area are well within minimum LOS range (approx.~140 NM for typical cruise altitudes18--60~000 feet in class A controlled airspace). 
  \end{description}

For tower and terminal areas, the LOS range is 58 and 118,5 NM, respectively.  With a maximum speed of 250 knots, this results in minimum time in LOS for approaching aircraft of 13,9 and 28,4 min, respectively. 
  For ACC, the LOS range is 140 NM for aircraft in Class A airspace, which at an unrestricted max cruise speed of 450 knots, results in a minimum time in LOS range of 18,6 min.
As was the case with TCAS, in all of these cases, these LOS range transition times are widely sufficient for the ADS-B receiver to receive Type B2 and C packets with high probability, even considering the packet loss probabilities for those distances, as shown in Table~\ref{tab:ATC}.

As for the uncertainty delay created by the reception of the interval keys, in the case of tower and terminal areas, these are 3,0 and 4,1 s respectively, which compares very favourably with the refresh rate of typical Secondary Surveillance Radar (SSR) installations used for ATC (6 antenna rotations per minute, resulting a 10 s refresh period).  The worst case here is that of the ACC, where the delay can be up to 14 sec, which remains comparable to the delay found in traditional radar-based infrastructures.


\begin{table}[ht]
    \begin{tabular}{|c||c|c|c|c||c|c|}%{|l|l|c|c|c|}
      \hline
      \textbf{ATC} & \textbf{radius} & $p$ (\%) & $\Delta_u(T_{B1})$ (s) & \textbf{update} (s) & \textbf{LOS} (min) &$\Delta_u(T_C)$ (s)\\
      \hline
        Tower & 5 NM     & 2,8 & 3,0 & 10 & 13,9 & 16,3  \\
              & (9,3 Km) &     &     &    &      &       \\
        \hline
        Terminal & 5--40 NM       & 22,2 & 4,1 & 10 & 28,4 & 25,0 \\
                 & (9,3--74,1 Km) &      &     &    &      & \\
        \hline
        ACC & 100--150 NM       & 83,3 & 14,0 & 10 & 18,6 & 82,1 \\
            & (185,2--277,8 Km) &      &      &    &      & \\
        \hline
    \end{tabular}
    \caption{Packet loss probability and uncertainty times for ATC.
      We give the \emph{radius} for the corresponding control area,
      the derived probability $p$ of packet loss, the expected
      authentication delay for interval key reception
      $\Delta_u(T_{B1})$, and compare it with the typical radar update
      rate.  We also compare the time in the LOS range with the
      expected uncertainty delay for Type C packet reception
      $\Delta_u(T_c)$.  We use the same parameters as before,
      i.e.~$T_{B1}=5$ s and $T_{B2}=T_C=30$ s.}
    \label{tab:ATC}
\end{table}

==> tableComparison.tex <==
\begin{table*}[ht!]
\centering
 \begin{tabular}{ |l |l | l | l | c | c | }
    \hline
     \multicolumn{2}{|c|}{Type} & Content & Period & \multicolumn{2}{c|}{Size (bits)} \\\cline{1-2}\cline{5-6}
     \multicolumn{1}{|c|}{SAT} & \multicolumn{1}{c|}{CABBA} & & & \multicolumn{1}{c|}{SAT} &  \multicolumn{1}{c|}{CABBA} \\\hline
%
     A & A & ADS-B message, MAC, sequence no. & \hfil - & 136 & 112\\\hline
%
     B & & Interval key & $T_{B}$ & 184 & - \\ \hdashline
       & B1 & Interval key & $T_{B1}$ & - & 112 \\ 
       & B2 & Interval key and signature & $T_{B2}$ & -  &  210 \\ \hline
     C & & \parbox[t]{5cm}{Interval key and signature; \\ aircraft public key and signature} &$T_C$ & 1520 &-\\ \hdashline
       & C & Aircraft public key and signature & & - & 242 \\
     \hline
    \end{tabular}
 \caption{A comparison of SAT and CABBA messages.  In CABBA, Type B messages are replaced with Type B1 messages at the beginning of each interval (each $T_B=T_{B1}$ seconds) and by Type B2 messages every $T_{B2}$ seconds.  Type C messages are shorter than in SAT and sent with period $T_C$.}
 \label{tab:CABBApacketTypes}
\end{table*}

==> tableImpactunAuth.tex <==
\begin{table}[h]
    \hskip-3.5cm
    \begin{tabular}{|l|l|c|c|c|c|c|c|c|c|c|}
        \hline
        & &  \textbf{P1}  & $\Delta_u(T_{B1})$& $\Delta_u(T_{B2})$&\textbf{P2} &$\Delta_u(T_{B1})$& $\Delta_u(T_{B2})$&  \textbf{P3}& x & q \\
        \hline
         \textbf{TCAS}& TA & 65.96 & 10.14 & 60.89 & 34.36 & 5.39 & 32.39 & 8.9 & 3.02 & 18.14 \\
        & RA & 65.80 & 10.11 & 60.71 & 33.56 & 5.30 & 31.82 & 6.4 & 2.86 & 17.16 \\
        \hline
         \textbf{ATC}& Tower & 65.55 & 10.07 & 60.44 & 32.36 & 5.16 & 30.99 & 2.8 & 2.64 & 15.88 \\
        & Terminal control area 1 & 65.74 & 10.10 & 60.65 & 33.27 & 5.27 & 31.62 & 5.5 & 2.80 & 16.83 \\
        & Terminal control area 2 & 66.87 & 10.32 & 61.89 & 38.74 & 5.93 & 35.62 & 22.2 & 4.10 & 24.61 \\
        & Area control center & 71.01 & 11.09 & 66.55 & 58.81 & 8.89 & 53.39 & 83.34 & 13.61 & 81.67 \\
        \hline
    \end{tabular}
    \caption{Summary of Parameters for TCAS and Controller Areas}
    \label{tab:parameters}
\end{table}


